Classification of tensor decompositions for II$_1$ factors

In the mid thirties Murray and von Neumann found a natural way to associate a von Neumann algebra $L(\Gamma)$ to any countable discrete group $\Gamma$. Classifying $L(\Gamma)$ in term of $\Gamma$ is a notoriously complex problem as in general the initial data tends to be lost in the von Neumann algebraic regime. An important problem in the theory of von Neumann algebras is to completely describe all possible tensor decompositions of a given group von Neumann algebra $L(\Gamma)$. In this direction the main goal is to investigate how exactly a tensor decomposition of $L(\Gamma)$ relates to the underlying group $\Gamma$. In this dissertation we introduce several new classes of groups $\Gamma$ for which all tensor decompositions of $L(\Gamma)$ are parametrized by the canonical direct product decompositions of $\Gamma$. Specifically, we show that whenever $L(\Gamma)\cong M_1\bar\otimes M_2$ where $M_i$ are any diffuse von Neumann algebras then there exists a non-canonical direct product decomposition $\Gamma=\Gamma_1\times\Gamma_2$ such that up to amplifications we have that $M_1\cong L(\Gamma_1)$ and $M_2\cong L(\Gamma_2)$. Our class include large classes of icc (infinite conjugacy class) amalgamated free products and wreath product groups. In addition we obtain similar classifications of tensor decompositions for the von Neumann algebras associated with the $T_0$ and $T_1$ group functors introduced by McDuff in $1969$.

==> thesisAbstract.tex <==



In the mid thirties Murray and von Neumann found a natural way to associate a von Neumann algebra $L(\Gamma)$ to any countable discrete group $\Gamma$.  Classifying $L(\Gamma)$ in term of $\Gamma$ is a notoriously complex problem as in general the initial data tends to be lost in the von Neumann algebraic regime. An important problem in the theory of von Neumann algebras is to completely describe all possible tensor decompositions of a given group von Neumann algebra $L(\Gamma)$. In this direction the main goal is to investigate how exactly a tensor decomposition of $L(\Gamma)$ relates to the underlying group $\Gamma$. 

In this dissertation we introduce several new classes of groups $\Gamma$ for which all tensor decompositions of $L(\Gamma)$ are parametrized by the canonical direct product decompositions of $\Gamma$. Specifically, we show that whenever $L(\Gamma)\cong M_1\bar\otimes M_2$ where $M_i$ are any diffuse von Neumann algebras then there exists a non-canonical direct product decomposition $\Gamma=\Gamma_1\times\Gamma_2$ such that up to amplifications we have that $M_1\cong L(\Gamma_1)$ and $M_2\cong L(\Gamma_2)$. Our class include large classes of icc (infinite conjugacy class) amalgamated free products and wreath product groups. In addition we obtain similar classifications of tensor decompositions for the von Neumann algebras associated with the $T_0$ and $T_1$ group functors introduced by McDuff in $1969$.     
 

==> thesisAbstractpublic.tex <==
In the study of tensor decomposition of von Neumann algebra, Popa introduced the notion of primeness which is analogous to prime numbers. However, the unique prime factorization of von Neumann algebras are much more complicated.  In our work we consider von Neumann algebra arising from a group and we obtain many new classes of groups $\Gamma$ that satisfy this classification result. This includes large families of amalgamated free products,  wreath products, McDuff’s groups. 


==> thesisAck.tex <==
First of all I am thankful to the Development and Promotion of Science and Technology Talents Project (DPST) in Thailand for the financial support and to my family for their love and encouragement.

I also thank Raul Curto, Victor Camillo, Palle Jorgensen, and Surjit Khurana for their time and serving on my dissertation committee


And last but not least, I would like to express my sincerest gratitude to my advisor Ionut Chifan for introducing me the research area and providing me opportunities with his kindness and support during my academic journey.
In addition as an advisee, I want to thank him for being a forgiver when I made mistakes, being a navigator when I lost my ways, being an excellent role model and showing me what a great mathematician should be with his passion in mathematics, and finally thank for being my advisor. 
